Denotational reasoning for asynchronous multiparty session types

We provide the first denotational semantics for asynchronous multiparty session types with precise asynchronous subtyping. Our semantics enables us to reason about asynchronous message-passing, in which message-sending is non-blocking. It enables us to prove the correctness of communication optimisations, in particular, those involving reordering of messages. Our development crucially relies on modelling message-passing as a computational effect. We apply grading, a paradigm for tracking computational effects, to asynchronous message-passing, demonstrating that multiparty session typing can be viewed as an instance of grading. We demonstrate the utility of our model by showing that it forms an adequate denotational semantics for a call-by-value asynchronous message-passing calculus, that ensures communication safety, deadlock-freedom and liveness in the presence of communication optimisations.

==> macros.tex <==
\makeatletter
\newlength\spacing@length
\DeclareRobustCommand\measure@width[1]{
\ifmmode\settowidth\spacing@length{$#1$}
\else\settowidth\spacing@length{#1}
\fi}
\newlength\spacing@length@
\DeclareRobustCommand\measure@width@[1]{
\ifmmode\settowidth\spacing@length@{$#1$}
\else\settowidth\spacing@length@{#1}
\fi}
\newcommand{\max@width}[2]{
\measure@width{#1}
\measure@width@{#2}
\ifthenelse{\spacing@length@ > \spacing@length}
{\setlength\spacing@length\spacing@length@}{}}
\newcommand{\padmathl}[2]{
\max@width{#1}{#2}
\mathrlap{#1}
\hspace{\spacing@length}}
\newcommand{\padmathc}[2]{
\max@width{#1}{#2}
\hspace{0.5\spacing@length}
\mathclap{#1}
\hspace{0.5\spacing@length}}
\newcommand{\padmathr}[2]{
\max@width{#1}{#2}
\hspace{\spacing@length}
\mathllap{#1}}
\makeatother



\newcounter{sarrow}
\newcommand{\xrightsquigarrow}[1]{%
\stepcounter{sarrow}%
\mathrel{\begin{tikzpicture}[baseline= {( $ (current bounding box.south) + (0,-0.5ex) $ )}]
  \node[inner sep=.6ex] (\thesarrow) {$\scriptstyle #1$};
  \path[draw,<-,decorate,
  decoration={zigzag,amplitude=0.7pt,segment length=1.0mm,pre=lineto,pre length=0.5pt}]
  (\thesarrow.south east) -- (\thesarrow.south west);
\end{tikzpicture}}%
}



\newcommand{\xleftrightarrows}[1]{\overset{#1}{\leftrightarrows}}

\newcommand{\rolecolor}{green!40!black}
\newcommand{\role}[1]{{\color{\rolecolor}{\mathsf{#1}}}}
\newcommand{\pp}{{\role{p}}}
\newcommand{\pq}{{\role{q}}}
\newcommand{\pr}{{\role{r}}}
\newcommand{\ps}{{\role{s}}}

\newcommand{\basetype}{\mathsf{b}}
\newcommand{\unittype}{\syntaxkeyword{unit}}
\newcommand{\booltype}{\syntaxkeyword{bool}}
\newcommand{\inttype}{\syntaxkeyword{int}}
\newcommand{\gto}[1]{\xrightarrow{#1}}

\newcommand{\msg}[2]{(#1, #2)}
\newcommand{\ml}[1]{\mathtt{#1}}
\newcommand{\mltype}[2]{#1 \langle #2 \rangle}
\newcommand{\sty}[1]{\mathbb{#1}}
\newcommand{\str}[1]{\mathsf{#1}}
\newcommand{\gty}[1]{\mathbb{#1}}

\newcommand{\ltypeend}{\mathsf{end}}
\newcommand{\ltypesend}[5]{\role{#1} \oplus_{#5} \mltype{#2}{#3}.\,#4}
\newcommand{\ltyperecv}[5]{\role{#1} \mathbin{\&}_{#5} \mltype{#2}{#3}.\,#4}
\newcommand{\ltypesendone}[4]{\role{#1} \oplus \mltype{#2}{#3}.\,#4}
\newcommand{\ltypesendoneprefix}[3]{\role{#1} \oplus \mltype{#2}{#3}}
\newcommand{\ltyperecvone}[4]{\role{#1} \mathbin{\&} \mltype{#2}{#3}.\,#4}
\newcommand{\ltyperecvoneprefix}[3]{\role{#1} \mathbin{\&} \mltype{#2}{#3}}
\newcommand{\ltypesendcases}[2]{\role{#1} \oplus \begin{cases}#2\end{cases}}
\newcommand{\ltyperecvcases}[2]{\role{#1} \mathbin{\&} \begin{cases}#2\end{cases}}
\newcommand{\ltyperec}[2]{\mu #1.\,#2}
\newcommand{\ltypevar}[1]{\mathsf{#1}}

\newcommand{\subst}[2]{#1[#2]}

\newcommand{\unfold}[1]{\mathcal{U}(#1)}
\newcommand{\typetree}[1]{\mathcal{T}(#1)}

\newcommand{\nconfigsymbol}{\mathcal{N}}
\newcommand{\nconfig}[1]{\mathcal{N}#1}
\newcommand{\mktree}[1]{\mathrm{tree}(#1)}
\newcommand{\nftree}[2]{\mathrm{nf}_{#1}(#2)}

\newcommand{\treegmonad}{\mathcal{N}}
\newcommand{\srgmonad}[2]{\mathrm{CT}_{#1}#2}
\newcommand{\return}{\mathrm{return}}
\newcommand{\bind}{\gg\!\!=}
\newcommand{\gbind}[2]{\overset{#1, #2}{\gg\!\!=}}
\newcommand{\effunit}{\ltypeend}
\newcommand{\effmul}{\cdot}
\newcommand{\effleq}[1][]{\subtype}

\newcommand{\compose}{\circ}
\renewcommand{\exp}[2]{#1 \Rightarrow #2}

\newcommand{\prectypesymbol}{{\prec}}
\newcommand{\prectype}[2]{#1 \prec #2}
\newcommand{\reduceinternalsymbol}{\xhookrightarrow{!}}
\newcommand{\reduceinternal}[5]{#1 \xhookrightarrow{#3 ! \mltype{#4}{#5}} #2}
\newcommand{\reduceexternalsymbol}{\xhookrightarrow{?}}
\newcommand{\reduceexternal}[5]{#1 \xhookrightarrow{#3 ? \mltype{#4}{#5}} #2}
\newcommand{\MaySend}[1]{\mathrm{MaySend}_{#1}}
\newcommand{\MayRecv}[1]{\mathrm{MayRecv}_{#1}}
\newcommand{\Sends}[1]{\mathrm{Sends}_{#1}}
\newcommand{\Recvs}[1]{\mathrm{Recvs}_{#1}}

\newcommand{\emptycontext}{\cdot}
\newcommand{\valuetypedg}[3]{#1 \vdash^{\mathtt{v}} #2 : #3}
\newcommand{\comptypedg}[6]{#1 \fatsemi #2 \fatsemi #3 \vdash #4 : #5 \fatsemi #6}
\newcommand{\conftypedg}[3]{\vdash #1 : #2 \fatsemi #3}

\newcommand{\rctx}[1]{\mathcal{#1}}
\newcommand{\hole}{\square}

\newcommand{\Result}{\mathrm{Result}}

\newcommand{\lambdasmp}{\ensuremath{\texttt{SafeMP}}}

\makeatletter
\newcommand{\lit}[1]{\mathord{\mathpalette\lit@{#1}}}
\newcommand{\lit@}[2]{%
  \mbox{%
    \scalebox{0.9}{%
      \ensuremath{#1\operatorname{\text{\sffamily\bfseries#2}}}%
    }%
  }%
}
\makeatother

\newcommand{\syntaxkeyword}[1]{\lit{#1}}

\newcommand{\unitterm}{\star}
\newcommand{\trueterm}{\syntaxkeyword{true}}
\newcommand{\falseterm}{\syntaxkeyword{false}}
\newcommand{\subtractterm}[2]{#1 - #2}
\newcommand{\addterm}[2]{#1 + #2}
\newcommand{\lessterm}[2]{#1 < #2}
\newcommand{\ifterm}[3]{\syntaxkeyword{if}~#1~\syntaxkeyword{then}~#2~\syntaxkeyword{else}~#3}
\newcommand{\absterm}[2]{\lambda #1.\,#2}
\newcommand{\letrecterm}[4]{\syntaxkeyword{let}~\syntaxkeyword{rec}\,#1 #2 = #3~\syntaxkeyword{in}~#4}
\newcommand{\recterm}[3]{\syntaxkeyword{rec}\,{#1}\,#2.\,#3}
\newcommand{\returntermkeyword}{\syntaxkeyword{return}}
\newcommand{\returnterm}[1]{\syntaxkeyword{return}\,#1}
\newcommand{\bindterm}[3]{\syntaxkeyword{let}~#1 = #2~\syntaxkeyword{in}~#3}
\newcommand{\letparterm}[2]{\syntaxkeyword{let}~#1~\syntaxkeyword{in}~#2}
\newcommand{\forktermkeyword}{\syntaxkeyword{fork}}
\newcommand{\forkterm}[2]{\syntaxkeyword{fork}~#1~\syntaxkeyword{with}~#2}
\newcommand{\applyterm}[2]{#1\,#2}
\newcommand{\sendtermkeyword}{\syntaxkeyword{send}}
\newcommand{\sendterm}[4]{\sendtermkeyword\,\msg{#1}{#2}\,\syntaxkeyword{to}\,\role{#3}\,\syntaxkeyword{then}\,#4}
\newcommand{\recvtermkeyword}{\syntaxkeyword{recv}}
\newcommand{\longrecvterm}[2]{\recvtermkeyword\,#1\,\{#2\}}
\newcommand{\recvterm}[5]{\longrecvterm{\role{#1}}{\mltype{#2}{#3}.\,#4}_{#5}}
\newcommand{\runsessionterm}[1]{\syntaxkeyword{run}{#1}}

\newcommand{\refines}{\lesssim}
\newcommand{\subtype}{\mathbin{<\vcentcolon}}
\newcommand{\notsubtype}{\mathbin{\not<\vcentcolon}}
\newcommand{\eqtype}{\equiv}
\newcommand{\suptype}{\mathbin{\vcentcolon>}}
\newcommand{\intleq}{\subtype^{\oplus}}
\newcommand{\intgeq}{\suptype^{\oplus}}
\newcommand{\extgeq}{\suptype^{\&}}
\newcommand{\asyncleq}{\subtype^{\mathsf{a}}}
\newcommand{\asyncgeq}{\suptype^{\mathsf{a}}}

\newcommand{\SO}{\mathrm{SO}}
\newcommand{\SI}{\mathrm{SI}}
\newcommand{\SISO}{\mathrm{SISO}}
\newcommand{\soset}[1]{\llparenthesis #1 \rrparenthesis_{\SO}}
\newcommand{\siset}[1]{\llparenthesis #1 \rrparenthesis_{\SI}}
\newcommand{\actset}[1]{\mathrm{act}(#1)}

\newcommand{\treeend}{\mathtt{0}}
\newcommand{\treereturnkeyword}{\mathtt{return}}
\newcommand{\treereturn}[1]{\treereturnkeyword(#1)}
\newcommand{\treesendkeyword}{\mathtt{send}}
\newcommand{\treesend}[3]{\treesendkeyword_{\role{#1}, #2} (#3)}
\newcommand{\treerecvkeyword}{\mathtt{recv}}
\newcommand{\treerecv}[3]{\treerecvkeyword_{\role{#1}} (#2)_{#3}}
\newcommand{\treeerror}{\mathtt{error}}

\newcommand{\hastype}[2]{#1 \blacktriangleleft #2}

\newcommand{\namepart}[2]{#1 \lhd #2}

\newcommand{\queue}[1]{\role{#1}}
\newcommand{\queueempty}{\emptyset}
\newcommand{\queueconcat}{\cdot}
\newcommand{\queueelem}[2]{\namepart{#1}{#2}}
\newcommand{\queuecong}{\equiv}
\newcommand{\dequeue}[2]{\mathrm{dequeue}_{#1}(#2)}
\newcommand{\inqueue}[2]{\langle #1, #2 \rangle}
\newcommand{\consfront}[3]{(\namepart{#1}{#2}) \dblcolon #3}
\newcommand{\consback}[3]{#1 \dblcolon (\namepart{#2}{#3})}
\newcommand{\config}[3]{(#1, #2, #3)}
\newcommand{\configcong}{\equiv}

\newcommand{\bisim}{\sim}

\newcommand{\sem}[2][]{#1{\left\llbracket #2 \right\rrbracket}}

\newcommand{\gtypeend}{\mathsf{end}}
\newcommand{\gtypecommone}[5]{\role{#1} \to \role{#2} \colon #3\langle #4 \rangle.\,#5}
\newcommand{\gtypecomm}[6]{\role{#1} \to \role{#2} \colon \{#3\langle #4 \rangle.\,#5\}_{#6}}
\newcommand{\gtypecommcases}[3]{\role{#1} \to \role{#2} \colon\mspace{-5mu} \begin{cases}#3\end{cases}}
\newcommand{\gtypevar}[1]{\mathsf{#1}}
\newcommand{\gtyperec}[2]{\mu #1.\, #2}


\newcommand{\tauaction}{\tau}
\newcommand{\sendaction}[2]{\role{#1}!#2}
\newcommand{\recvaction}[2]{\role{#1}?#2}
\newcommand{\commaction}[3]{\role{#1} \to \role{#2} : #3}

\newcommand{\reducesymbol}{\rightsquigarrow}
\newcommand{\reduceaction}[3]{#1 \xrightsquigarrow{\padmathc{#3}{\mspace{8mu}}} #2}
\newcommand{\reduceactionmany}[3]{#1 \mathbin{{\xrightsquigarrow{\padmathc{#3}{\mspace{8mu}}}}{}^*} #2}

\newcommand{\RuleName}[1]{\text{\rm\scriptsize{\color{green!40!black}{[\textsc{#1}]}}}}
\newcommand{\TRULE}[1]{\RuleName{#1}}

\newcommand{\project}[2]{#1 \upharpoonright #2}
\newcommand{\rproject}[3]{#1 \downharpoonleft_{#2} #3}
\newcommand{\rprojectmerge}[3]{#1 \downharpoonleft'_{\role{#2}} #3}
\newcommand{\bmergeltype}{\sqcap}
\newcommand{\mergeltype}[2]{{\textstyle\bigsqcap_{#2} #1}}
\newcommand{\bcomergeltype}{\sqcup}
\newcommand{\comergeltype}[2]{{\textstyle\bigsqcup_{#2} #1}}
\newcommand{\pactive}[2]{\mathrm{active}_{#2}(#1)}
\newcommand{\pinactive}[2]{\mathrm{inactive}_{#2}(#1)}
\newcommand{\psynchronous}[2]{\mathrm{synchronous}_{#2}(#1)}
\newcommand{\swap}[3]{(\role{#1} \leftrightarrows \role{#2})\, \role{#3}}
\newcommand{\swapinset}[3]{\swap{#1}{#2}{#3}}
\newcommand{\Conforms}[3]{\mathsf{Conf}_{#1}{(#2; #3)}}

\newcommand{\Label}{\mathcal{L}}

